ADL-ID: Adversarial Disentanglement Learning for Wireless Device Fingerprinting Temporal Domain Adaptation

As the journey of 5G standardization is coming to an end, academia and industry have already begun to consider the sixth-generation (6G) wireless networks, with an aim to meet the service demands for the next decade. Deep learning-based RF fingerprinting (DL-RFFP) has recently been recognized as a potential solution for enabling key wireless network applications and services, such as spectrum policy enforcement and network access control. The state-of-the-art DL-RFFP frameworks suffer from a significant performance drop when tested with data drawn from a domain that is different from that used for training data. In this paper, we propose ADL-ID, an unsupervised domain adaption framework that is based on adversarial disentanglement representation to address the temporal domain adaptation for the RFFP task. Our framework has been evaluated on real LoRa and WiFi datasets and showed about 24% improvement in accuracy when compared to the baseline CNN network on short-term temporal adaptation. It also improves the classification accuracy by up to 9% on long-term temporal adaptation. Furthermore, we release a 5-day, 2.1TB, large-scale WiFi 802.11b dataset collected from 50 Pycom devices to support the research community efforts in developing and validating robust RFFP methods.

==> experiment.tex <==
We use our testbed described in Section~\ref{sec:testbed} to create and collect large-scale, comprehensive LoRa RF fingerprinting dataset for multiple experimental scenarios that are specifically designed to allow intensive and comprehensive performance evaluation of various deep learning-based wireless networks techniques, with a special focus on RF/device fingerprinting. We chose a bandwidth of $125$KHz for all LoRa transmissions. However, in \cite{elmaghbub2020widescan}, we demonstrated that considering out of band spectrum enhances the performance of the model, and hence we provide a total bandwidth of $1$MHz that covers the in-band as well as an adjacent out of band spectrum of LoRa transmissions for all setups. In the remainder of this section, we present each of the seven considered experimental setups. Throughout this section, we will be referring to Fig.~\ref{fig:flow1} for experimental setups 1, 2, and 3, and for Fig.~\ref{fig:flow2} for experimental setups 4, 5, 6 and 7. Table~\ref{summary} summarizes these 7 setups.
%Each scenario comprises multiple transmissions of each transmitter. 
%We created raw-IQ and FFT-based representation files for each transmission in ".dat" format.


\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/Scen_a.pdf}
    \caption{Setup diagram: setups 1, 2 and 3.}
    \label{fig:flow1}
\end{figure}

\subsection{Setup 1: Different Days Indoor Scenario}
%To mask the impact of the outside weather and 
In order to enable performance evaluation while masking the impact of the outside environment, we created an indoor setup, ran experiments, and collected datasets for this setup. These indoor experiments were carried out in a typical occupied room environment over $5$ consecutive days. All devices transmitted the same message from the same location, $5$m away from the receiver so that all devices experience similar channel conditions. As shown in Fig.~\ref{fig:flow1}, for each day, each transmitter generated $10$ transmissions, each of $20$s duration, all spaced apart by $1$ minute. Hence, we collected about $200$M complex-valued samples from each device per day. We used GNURadio packages to store the sampled raw-I/Q values and their corresponding FFT-Based representation into binary files as depicted in Fig.~\ref{fig:flow1}.

\subsection{Setup 2: Different Days Outdoor Scenario}
%For millions of outdoor LoRa-enabled sensors, it is more realistic also to include an outdoor setup to examine the impact of outdoor wireless channel impairments. 
In order to allow for performance evaluation while considering the impact of outdoor wireless channel impairments, we carried out the experiments in an outdoor environment at nighttime. Here again, all devices transmitted the same message from the exact location, situated $5$m away from the receiver, so that all devices experience similar channel conditions. Like in the indoor setup case and as shown in Fig.~\ref{fig:flow1}, for five consecutive days, each transmitter generated $10$ transmissions per day, each of $20$s duration, all spaced $1$ minute apart from one another. This resulted in about $200$M complex-valued samples per device per day. We ran this experiment over $5$ consecutive days and provided 5-day worth of data to study the robustness of deep learning models when trained on data collected on one day but tested on data captured on a different day.  We used GNURadio packages to store the sampled raw-I/Q values and their corresponding FFT-based representation into binary files as depicted in Fig.~\ref{fig:flow1}.

\subsection{Setup 3: Different Days Wired Scenario} The wireless channel has a notable impact on the performance of deep learning models and presents its unique challenges \cite{al2020exposing}. Hence, to assess how well these models perform in the absence of the wireless channel's impact, we created a wired setup where the Pycom boards are directly connected to the USRP via an SMA cable and $30$dB attenuator. Similar to the Indoor and Outdoor experiments, we ran this experiment over $5$ consecutive days. For every day, each device transmitted $10$ bursts each of $20$s duration. Therefore, the total amount of collected data is $200$M complex-valued samples per device per day. We again used GNURadio packages to store the sampled raw-I/Q values and their corresponding FFT-based representation into binary files as depicted in Fig.~\ref{fig:flow1}.

\subsection{Setup 4: Different Distances Scenario}
Some end-devices constantly change their positions, so it is critical to explore the impact of distance on the performance of classifiers and see whether or not a classifier would still recognize a device when it moves to a position that is different from the one used for training. This experiment was carried out in a typical outdoor environment in a sunny day. We considered four different distances, $5$m, $10$m, $15$m, and $20$m, and for each distance, we collected $1$ transmission of $20$s for each of the $25$ devices. We kept the receiver at the same location for all the transmissions while locating the transmitters at $4$ different distances away from the receiver base ($5$m, $10$m, $15$m, and $20$m). The transmissions were captured consecutively in time with only $60$s apart from one another. Each transmitter generated $4$ transmissions each of $20$s duration, resulting in $80$M complex-valued samples from each device. We again used GNURadio packages to store the sampled raw-I/Q values and corresponding FFT-based samples into binary files as depicted in Fig.~\ref{fig:flow2}.

\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{figures/scen_b2.pdf}
    \caption{Setup diagram: setups 4, 5, 6, and 7.}
    \label{fig:flow2}
\end{figure}

\subsection{Setup 5: Different Configurations Scenario}
LoRaWAN uses the Adaptive Data Rate (ADR) mechanism to optimize the data rates, air-time, and energy consumption in the network to accommodate the varying RF conditions. This mechanism allows the network server to inform end devices to adjust their power consumption and data rate as needed. This is achievable by controlling the following parameters at end devices: spreading factor, bandwidth, and power consumption. Changing the spreading factor, for example, in LoRa modulation results in a change in the data rate, receiver sensitivity, time in the air, and power consumption. Fig.~\ref{fig:spec4} shows the frequency spectrum of a snapshot of the four LoRa configurations that we included in our dataset. Ideally, a classification model (e.g., a deep learning fingerprinting model) should identify a device even if it changes its configuration; i.e., models that are trained using one configuration but tested on a different configuration should still perform well. Therefore, in order to enable the assessment of how agnostic these models are to protocol configuration, we captured transmissions using $4$ different configurations, as presented in Table~\ref{con}. For this, we collected a single LoRa transmission of $20$s from each device for each configuration in an indoor setup with $5$m as the distance between the receiver and transmitters. Like other setups, for this setup, we used GNURadio packages to store the sampled raw-I/Q values and their corresponding FFT-based representation into binary files as depicted in Fig.~\ref{fig:flow2}.
\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth,height=0.53\columnwidth]{figures/con_spec.pdf}
    \caption{Spectrum of the 4 LoRa configurations from Setup 5}
    \label{fig:spec4}
\end{figure}
\subsection{Setup 6: Different Locations Scenario}
Another practical scenario we consider here aims at allowing deep learning models to be trained on data captured in one location but tested on data collected in another location. For this, we captured LoRa transmissions in three different location deployments, room environment, office environment, and outdoor environment, all taken on the same day. Here, we kept the distance between the receiver and transmitters (i.e., $5$m) and the LoRa configuration the same. We captured a single transmission of $20$s from each device at each location with a $60$s period between the devices, resulting in $60$M complex samples from each device. We again used GNURadio packages to store the sampled raw-I/Q values and their corresponding FFT-based representation into binary files as depicted in Fig.~\ref{fig:flow2}.
\begin{table}
\scriptsize
%\begin{adjustbox}{width=1\columnwidth, height = 0.15\columnwidth, center}
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{tabular}{|l|c|c|l|c|c|}
\hline
\textbf{Configurations} & \multicolumn{1}{l|}{{ \textbf{\begin{tabular}[c]{@{}l@{}}Spread\\ Factor\end{tabular}}}} & \multicolumn{1}{l|}{{ \textbf{Bandwidth}}} & \textbf{Bit Rate} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Tx \\ Power\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Coding\\ Rate\end{tabular}}} \\ \hline
Configuration 1 & { 7}                                                                                     & {\color[HTML]{333333} 125KHz}                                  & 5470 bps          & 20dBm                                                                              & 4/5                                                                                 \\ \hline
Configuration 2 & 8                                                                                                            & 125KHz                                                         & 3125 bps          & 20dBm                                                                              & 4/5                                                                                 \\ \hline
Configuration 3 & 11                                                                                                           & 125KHz                                                         & 537 bps           & 20dBm                                                                              & 4/5                                                                                 \\ \hline
Configuration 4 & 12                                                                                                           & 125KHz                                                         & 293 bps           & 20dBm                                                                              & 4/5                                                                                 \\ \hline
\end{tabular}
%\end{adjustbox}

\caption{LoRa Configurations}
\label{con}

\end{table}

\subsection{Setup 7: Different Receivers Scenario}
Like transmitters, receivers also suffer from hardware impairments due to hardware imperfection. Therefore, deep learning models trained using data collected by one receiver but tested using data collected by a different receiver may not perform well due to the possible additional impairments caused by the receiver's reception.
To allow researchers to study the impact of such a change in the receiving device, we provided a dataset for the 25 Pycom transmitting devices, collected using two different USRP B$210$ receivers. In this experiment,  we considered an indoor setup where the transmitters (the 25 Pycom devices) were located $5$m away from the receiver. For each receiver, we captured a single transmission of $20$s from each of the 25 Pycom transmitters, yielding a total of $40$M samples for each device. Like other setups, for this setup, we used GNURadio packages to store the sampled raw-I/Q values and their corresponding FFT-based representation into binary files as depicted in Fig.~\ref{fig:flow2}.

==> intro_copy.tex <==
This paper presents and releases a comprehensive dataset consisting of massive RF signal data captured from $25$ LoRa-enabled transmitters using Ettus USRP B$210$ receivers. The RF dataset provides the research community with a set of first-of-its-kind real-world setups, all helpful in enabling the study of the effectiveness and robustness of deep learning-based wireless techniques, such as RF/device fingerprinting. These experimental setups cover and provide a comprehensive set of practical scenarios for indoor and outdoor environments while considering various realistic network deployment variability across time, location, hardware, and modulation configuration. These are obtained by varying network deployment and configuration parameters, such as the distance between the transmitters and the receiver, the configuration of the LoRa protocol, the physical location of the experiment, and the receiver hardware used for collecting the data samples and for training/testing the neural network models.
%I think the text here is a little bit confusing. 
%I suggest we say: (for collecting the data samples for training ...) because not the receiver hardware itself has been used for training and testing (which is the server) but rather we mean the data captured by the receiver which used for the training and inference stages. 

As research communities move away from model-based to data-driven solutions, many recently proposed frameworks on device/RF fingerprinting have also shifted from model-based classification approaches to deep learning-based approaches. Although recently proposed deep learning-based approaches have shown promising results, %most of them (with the exception of a few) rely on synthesized data for evaluation and validation 
some still rely on synthesized data for evaluation and validation, and most of those that rely on real datasets are evaluated on general indoor and outdoor setups, leaving behind many questions that need to be answered before claiming the feasibility and superiority of their proposed techniques in real-world settings. 

Other essential experimental scenarios, which are very useful for assessing the capability and robustness of deep learning-based fingerprinting techniques, have not been investigated. These essential scenarios allow for the study of the impact of various deployment parameters on the performances achievable by these techniques, such as the impact of the distance between the transmitters and the receiver, the configuration of the used protocol, the physical location of the conducted measurements, and the hardware impairments of the receiver used in the training and inference stages. %\hl{used for training and testing the deep learning models. }
%suggestion: used to capture the training and testing data for the deep learning models."


%Also, it is crucial to investigate the dependency of the trained models on the hardware impairments of the receivers used for collecting the training dataset. 
Another important scenario that is also missing is the study of the performance of deep learning models when the RF signals are captured during concurrent transmissions where some portions of the incoming packets overlap.  
 
A major challenge the wireless research community has been facing is the lack of comprehensive, publicly available datasets that could serve as benchmarks for the device/RF classification and fingerprinting techniques \cite{al2020exposing}. 
Having public and easily accessible dataset benchmarks has indeed been one of the main drivers for innovation and idea maturity in closely related fields, like image recognition and natural language processing, in addition to creating collaboration opportunities among researchers. Therefore, such efforts must be mimicked in the wireless community to be able to foster innovation in this domain as well.
%Fortunately, recently, researchers from Northeastern University released their collected IEEE 802.11 a/g (WiFi) dataset and made it accessible to the public for use, thus making a good step in this regard~\cite{al2020exposing}.

%to help to solve the issue and spreading the new culture.
 
 \subsection{What Distinguishes Our Dataset From Existing Ones?}
 %\bh{Outline of this sectcion\\
 %-Talk about recent RF datasets\\
 %- Talk about what do these existing datasets fail to offer: e.g., not providing comprehensive scenarios, WiFi, no LoRa, Out of band, etc.\\
 %- Say what is unique about our dataset}
 
Researchers in \cite{aernouts2018sigfox} presented three LPWAN (Sigfox and LoRAWAN) datasets collected in an outdoor environment aimed at evaluating location fingerprinting algorithms. These datasets have been collected over three months in both rural and urban areas.
Sigfox-rural and Sigfox-urban datasets consist respectively of $25$k+ and $14$k+ Sigfox messages, whereas LoRaWAN dataset consists of $123$k+ LoRaWAN messages. These messages include a couple of protocol information, time of reception, and GPS location information but do not include device labels, and therefore, can not be used for supervised deep learning-based device classification. The closest existing work to our work is the recently released work at Northeastern University~\cite{al2020exposing}, which collected and released a massive dataset of IEEE 802.11 a/g (WiFi) standard data obtained from 20 wireless devices with identical RF circuitry over several days in (a) an anechoic chamber, (b) in-the-wild testbed, and (c) with cable connections. The focus of the Northeastern dataset is to explore the impact of the wireless channel on the performance of deep learning-based RF fingerprinting models. The dataset is limited in terms of the covered scenarios, and it is for WiFi signals only. Unfortunately, to the best of our knowledge, there are still no public datasets for LoRa device fingerprinting nor datasets that include the diverse experimental scenarios we mentioned. Our dataset presented in this paper fulfills the need for a large-scale LoRa dataset covering a wide range of diverse scenarios for a more comprehensive evaluation and validation.  
 
      \begin{table*}
%\resizebox{18cm}{!}{
\begin{adjustbox}{width=2\columnwidth, height = 0.17\columnwidth, center}


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Setups}                                    & {\color[HTML]{333333} \textbf{\begin{tabular}[c]{@{}c@{}}Number of\\ Transmitters\end{tabular}}} & { \textbf{\begin{tabular}[c]{@{}c@{}}Number of\\  Receivers\end{tabular}}} & \textbf{Protocol} & \textbf{\begin{tabular}[c]{@{}c@{}}Number \\ of Days\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Transmissions \\ per Device\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Duration per \\ Transmission\end{tabular}} & \textbf{Distances} & \textbf{Environment} & \textbf{Representation} \\ \hline
{1) Diff Days Indoor}                              & {\color[HTML]{333333} 25}                                                                        & {\color[HTML]{333333} 1}                                                                       & LoRa              & 5             & 10                                                                           & 20s                                                                           & 5m                 & Indoor               & IQ/FFT                  \\ \hline
{2) Diff Days Outdoor}                             & 25                                                                                               & 1                                                                                              & LoRa              & 5             & 10                                                                           & 20s                                                                           & 5m                 & Outdoor              & IQ/FFT                  \\ \hline
{3) Diff Days Wired}                               & 25                                                                                               & 1                                                                                              & LoRa              & 5             & 10                                                                           & 20s                                                                           & 5m                 & Wired                & IQ/FFT                  \\ \hline
{4) Diff Distances}                            & 25                                                                                               & 1                                                                                              & LoRa              & 1             & 4                                                                            & 20s                                                                           & 5,10,15,20m        & Outdoor              & IQ/FFT                  \\ \hline
\multicolumn{1}{|l|}{{5) Diff Configurations}} & 25                                                                                               & 1                                                                                              & LoRa              & 1             & 4                                                                            & 20s                                                                           & 5m                 & Indoor               & IQ/FFT                  \\ \hline
{6) Diff Locations}                            & 25                                                                                               & 1                                                                                              & LoRa              & 1             & 3                                                                            & 20s                                                                           & 5m                 & 2 Indoor, 1 Outdoor  & IQ/FFT                  \\ \hline
{7) Diff Receivers}                            & 25                                                                                               & 2                                                                                              & LoRa              & 1             & 2                                                                            & 20s                                                                           & 5m                 & Indoor               & IQ/FFT                  \\ \hline
\end{tabular}

\end{adjustbox}
\caption{Summary of Experimental Setups/Scenarios.}
\label{summary}
\end{table*}

\subsection{Our LoRa Dataset in Brief}
Our RF dataset provides both time-domain I/Q samples and corresponding FFT samples collected using an IoT testbed consisting of $25$ identical Pycom IoT devices and a USRP B$210$ receiver, operating at a center frequency of $915$MHz, used for recording the received signals sampled at $1$MS/s. Recorded data in the form of both the time-domain I/Q samples and FFT samples are stored into binary files in compliance with SigMF~\cite{hilburn2018sigmf} by creating, for each binary file, a metafile written in plain-text JSON to include recording information such as sampling rate, time and day of recording, and carrier frequency, among other parameters. 

This dataset covers multiple experimental setup scenarios, which are summarized in Table \ref{summary} and can be downloaded at
\href{https://research.engr.oregonstate.edu/hamdaoui/datasets/}{\color{blue}{http://research.engr.oregonstate.edu/hamdaoui/datasets}}. 

The experimental scenarios are briefly described next, with more details provided in~\cite{elmaghbub2021lora}.
 \begin{itemize}
         \item {\bf Setup 1---Different Days Indoor Scenario:} Indoor setup with data collected over $5$ consecutive days. For each day, $10$ transmissions were captured from each of the 25 transmitters, with each transmission having a duration of $20$s. All transmissions took place $1$ minute apart from one another. 
         %About $200$M complex-valued samples of raw I/Q values and corresponding FFT-based representation are provided as binary files.
         \item {\bf Setup 2---Different Days Outdoor Scenario:} Outdoor setup with data collected over $5$ consecutive days. For each day, $10$ transmissions were captured from each of the $25$ transmitters, with each transmission having a duration of $20$s. All transmissions took place $1$ minute apart from one another. 
         %About $200$M complex-valued samples of raw I/Q values and corresponding FFT-based representation are provided as binary files. 
         \item {\bf Setup 3---Different Days Wired Scenario:} Wired setup with data collected over $5$ consecutive days. For each day, $10$ transmissions were captured from each of the $25$ transmitters, with each transmission having a duration of $20$s. All transmissions are $1$ minute apart from one another. 
         %About $200$M complex-valued samples of raw I/Q values and corresponding FFT-based representation are provided as binary files. 
         \item {\bf Setup 4---Different Distances Scenario:} Outdoor setup with data collected from $4$ different distances: $5$m, $10$m, $15$m, and $20$m away from the receiver. For each distance, one transmission was captured from each of the $25$ transmitters, with each transmission having a duration of $20$s. All transmissions are $1$ minute apart from one another. 
         %About $80$M complex-valued samples of raw I/Q values and corresponding FFT-based representation are provided as binary files. 
         \item {\bf Setup 5---Different Configurations Scenario:} Indoor setup with data collected from $4$ different LoRa configurations. For each configuration, one transmission was captured from each of the $25$ transmitters, with each transmission having a duration of $20$s. All transmissions are $1$ minute apart from one another. 
         %About $80$M complex-valued samples of raw I/Q values and corresponding FFT-based representation are provided as binary files.
         \item {\bf Setup 6---Different Locations Scenario:} This data has been collected in $3$ different locations: room, outdoor, and office environments. At each location, one transmission was captured from each of the $25$ transmitters, with each transmission having a duration of $20$s. All transmissions are $1$ minute apart from one another.
         %About $60$M complex-valued samples of raw I/Q values and corresponding FFT-based representation are provided as binary files. 
         \item {\bf Setup 7---Different Receivers Scenario:} Indoor setup with data collected using $2$ different receivers. For each receiver, one transmission was captured from each of the $25$ transmitters, with each  having a duration of $20$s. All transmissions are $1$ minute apart from one another. 
         %About $40$M complex-valued samples of raw I/Q values and corresponding FFT-based representation are provided as binary files. 
\end{itemize}
     

The rest of the paper is organized as follows. Section \ref{sec:testbed} describes the testbed components. Sections~\ref{experiment} and~\ref{dataset} describe the different experimental setups and the dataset, respectively. Section~\ref{use-case} presents a use case for the dataset. The challenges, limitations, and new opportunities are discussed in Section \ref{challenges} and the paper is concluded in Section \ref{Conclusion}. 
     
     
     

